Hyperparameter Optimization in Machine Learning

Hyperparameters are configuration variables controlling the behavior of machine learning algorithms. They are ubiquitous in machine learning and artificial intelligence and the choice of their values determines the effectiveness of systems based on these technologies. Manual hyperparameter search is often time-consuming and becomes infeasible when the number of hyperparameters is large. Automating the search is an important step towards advancing, streamlining, and systematizing machine learning, freeing researchers and practitioners alike from the burden of finding a good set of hyperparameters by trial and error. In this survey, we present a unified treatment of hyperparameter optimization, providing the reader with examples, insights into the state-of-the-art, and numerous links to further reading. We cover the main families of techniques to automate hyperparameter search, often referred to as hyperparameter optimization or tuning, including random and quasi-random search, bandit-, model-, population-, and gradient-based approaches. We further discuss extensions, including online, constrained, and multi-objective formulations, touch upon connections with other fields, such as meta-learning and neural architecture search, and conclude with open questions and future research directions.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit 
%Publisher 
authors'  
approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> com2.tex <==
\def\RSet{\mathbb{R}}
\def\NSet{\mathbb{N}}

\newcommand{\hmmax}{0}
\newcommand{\bmmax}{2} % https://www.texfaq.org/FAQ-manymathalph
% \usepackage[mathscr]{euscript}
\usepackage{bm}

\usepackage{tikz}
\usepackage{txfonts}
\usepackage{comment}
\usetikzlibrary{shapes,arrows}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}



\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmink}{arg\,min-k}
% big composition symbol
\makeatletter
\newcommand{\bigcomp}{%
  \DOTSB
  \mathop{\vphantom{\sum}\mathpalette\bigcomp@\relax}%
  \slimits@
}
\newcommand{\bigcomp@}[2]{%
  \begingroup\m@th
  \sbox\z@{$#1\sum$}%
  \setlength{\unitlength}{0.9\dimexpr\ht\z@+\dp\z@}%
  \vcenter{\hbox{%
    \begin{picture}(1,1)
    \bigcomp@linethickness{#1}
    \put(0.5,0.5){\circle{1}}
    \end{picture}%
  }}%
  \endgroup
}
\newcommand{\bigcomp@linethickness}[1]{%
  \linethickness{%
      \ifx#1\displaystyle \
       2\fontdimen8\textfont\else
      \ifx#1\textstyle 1.65\fontdimen8\textfont\else
      \ifx#1\scriptstyle 1.65\fontdimen8\scriptfont\else
      1.65\fontdimen8\scriptscriptfont\fi\fi\fi 3
  }%
}
% -----------------------------------------



\def\massi#1{\fxfatal[author=Massi]{#1}}
\newcommand{\Lagr}{\mathcal{L}}
\newcommand{\opt}{\textsc{(Optional) }}
\newcommand{\vx}{x}
\newcommand{\mw}{W}
%newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vlambda}{{\lambda}}
\newcommand{\vy}{y}
\newcommand{\vc}{c}
\newcommand{\mc}{C}
\newcommand{\vw}{w}
\newcommand{\vb}{b}
% \newcommand{\Lagr}{\mathcal{L}}
% \newcommand{\MP}[1]{\textcolor{blue}{#1}}
\newcommand{\lf}[1]{\textcolor{blue}{\textit{[#1]}}}
\newcommand{\mik}[1]{\textcolor{magenta}{#1}}
\def\transpose#1{#1^\intercal}
\newcommand{\pproc}[1]{\texttt{#1}}


\newcommand{\idfunc}{\mathrm{id}}


\newcommand{\inputdim}{n}
\newcommand{\outputdim}{c}
\newcommand{\datasetdim}{N}

\newcommand{\diracdelta}[1]{\delta_{#1}}

\newcommand{\diag}[1]{\mathrm{diag}(#1)}

\newcommand{\weightspace}{\mathcal{W}}


\usepackage{dsfont}
\def\RSet{\mathds{R}}
\def\Rset{\mathds{R}}
\def\QSet{\mathds{Q}}
\def\NSet{\mathds{N}}
\def\ZSet{\mathds{Z}}
\def\CSet{\mathds{C}}

\DeclareMathOperator{\E}{\mathds{E}}
\DeclareMathOperator{\expectation}{\mathds{E}}
\DeclareMathOperator{\Pro}{\mathds{P}}
% \DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\tr}{tr}
% \DeclareMathOperator{\diag}{diag}
\usepackage{commath} % For differentials, partial derivatives etc
\def\abk#1{\left\langle #1 \right\rangle}

% \usepackage{bm}
\newcommand{\vect}[1]{\boldsymbol{{#1}}}
% Bold upright symbols, including greek stuff
% http://tex.stackexchange.com/questions/3535/bold-math-automatic-choice-between-mathbf-and-boldsymbol-for-latin-and-greek
\def\ONE#1{\mathds{1}\!\left\{#1\right\}}
\def\transpose#1{#1^\mathsf{T}}
\def\bel#1{\mathrm{bel}\!\left\{#1\right\}}
\def\alert#1{\textit{#1}}

\usepackage{xcolor}
% \DeclareMathOperator{\argmin}{argmin}

\newcommand{\Prange}[2]{{P_{#1:\,#2}} }

\newcommand{\lds}{\textsc{LDS}\xspace}

\newcommand{\needcite}{\lf{need citations}}

% complexity bounds for AD
\newcommand{\workad}{\texttt{work}}
\newcommand{\taskad}{\texttt{task}}
\newcommand{\timead}{\texttt{time}}
\newcommand{\evalad}{\texttt{eval}}

% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% fundamentals
\newcommand{\inputspace}{\mathcal{X}}
\newcommand{\featurespace}{\mathcal{V}}
\newcommand{\outputspace}{\mathcal{Y}}
\newcommand{\function}{f}
% \newcommand{\expectation}{\mathbb{E}}
\newcommand{\innerloss}{L}
\newcommand{\outerloss}{E}
\newcommand{\loss}{\ell}
\newcommand{\valmetric}{\mathscr{M}}
\newcommand{\hypothesis}{h}
\newcommand{\hypothesisspace}{\mathcal{H}}
\newcommand{\jointprob}{p_{xy}}

\newcommand{\exprisk}{\mathcal{E}}
\newcommand{\emprisk}{\hat{\mathcal{E}}}

\newcommand{\hidden}{z}

%
\newcommand{\dotprod}[2]{\langle #1 , #2 \rangle}
\newcommand{\dimopthyper}{a}
\newcommand{\dimstate}{d'}
\newcommand{\opthyperspace}{A}

% hyperparamter optimization rev
\newcommand{\learningalgo}{A}

\usepackage[scr=rsfso]{mathalfa}
\newcommand{\setofdata}{\mathscr{D}}
% \newcommand{\setofdata}{\mathcal{D}}

% Parameters of the hyperparameter optimization algorithm 
\newcommand{\hpoap}{\upsilon}

\newcommand{\Dtrain}{\mathcal{D}}
\newcommand{\Dval}{\mathcal{V}}
\newcommand{\Dtest}{D_{\mathrm{ts}}}
\newcommand{\objtrain}{\mathcal{J}}


\newcommand{\surrogm}{\hat{f}}

% gb hpo 
\newcommand{\hypergrad}{g}
\newcommand{\onlinehypergrad}{\Tilde{g}}

% meta-learning
\newcommand{\metalalgo}{\mathbfcal{A}}
\newcommand{\metahyperparameters}{\boldsymbol{\lambda}}
\newcommand{\setofmetadata}{\mathbfcal{D}}
\newcommand{\metatrainset}{\mathbf{D}_{\operatorname{tr}}}
\newcommand{\metavalset}{\mathbf{D}_{\operatorname{val}}}
\newcommand{\metatestset}{\mathbf{D}_{\operatorname{ts}}}



\newcommand{\spaceoflearningalgo}{\mathbfcal{H}}
\newcommand{\metadataset}{\mathbf{D}}
\newcommand{\metadatasetdim}{\mathbf{N}}
\newcommand{\mtlexprisk}{\mathbfcal{E}}
\newcommand{\mtlemprisk}{\hat{\mathbfcal{E}}}
\newcommand{\task}{\tau}
\newcommand{\spaceoftasks}{\mathcal{T}}
\newcommand{\taskinmetadist}{\task}
\newcommand{\metadistr}{p_{D, \taskinmetadist}}
\newcommand{\metadistrr}{p_{\taskinmetadist, D}}
\newcommand{\metadistrrr}{p_{D}(\cdot|\taskinmetadist)p_{\taskinmetadist}}
\newcommand{\mtlhyperparamspace}{\mathbf{\Lambda}}

\newcommand{\genericdatasample}{\bar{D}}
\newcommand{\genericnumberofpoints}{\bar{N}}
\newcommand{\generictasksample}{\bar{\task}}
% \newcommand{\genericmetahpcomp}{\mathbf{h}}

\newcommand{\algoofalgos}{\hat{\learningalgo}}

% transfer learning
\newcommand{\sourcetask}{\task_{\mathrm{s}}}
\newcommand{\targettask}{\task_{\mathrm{t}}}
\newcommand{\sourcedata}{D_{\mathrm{s}}}
\newcommand{\targetdata}{D_{\mathrm{t}}}




% ---------- NEW ENVIRONMENTS ------------
%----------------------------------------------------------------

%\newcommand{\anres}{Theorem}
%\newtheorem{anresth}{\anres}

% ---------- NEW COMMAND DEFINITIONS ------------
% \DeclareMathAlphabeth{\mathcal}{OMS}{cmsy}{m}{n}

% for blank pages

\newcommand{\blankpage}{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}
    
    
%%%% IMPORTED FROM ITER_COMPLEX -----------------


% gradients and jacobians
\newcommand{\grad}{\nabla}
\newcommand{\jac}{\partial}
\newcommand{\hess}{\grad^2}

\newcommand{\Xs}{\mathcal{X}}
\newcommand{\Ys}{\mathcal{Y}}
\newcommand{\Zs}{\mathcal{Z}}



%Bilevel commands
\newcommand{\fo}{E} % outer function
\newcommand{\fin}{\ell} % inner function
\newcommand{\proj}{\mathcal{P}_\Lambda}

% bound constants
\newcommand{\Low}{\xi_{1,\lambda}}
\newcommand{\Lol}{\xi_{2,\lambda}}
\newcommand{\Bo}{\nu_{E,\lambda}}


% \newcommand{\D}{D_\lambda}


% contraction mapping constants
\newcommand{\q}{\rho_\lambda}
\newcommand{\supq}{q}
\newcommand{\rhol}{\nu_{2, \lambda}}
\newcommand{\rhow}{\nu_{1, \lambda}}
\newcommand{\LPhi}{{\nu}_{\Phi, \lambda}}

%algorithm rate
\newcommand{\rf}{\rho_\lambda}
\newcommand{\hrf}{\sigma_{\lambda}}




%lip, s.c. lower-level constants
\newcommand{\Llw}{L_\fin(\lambda)}
\newcommand{\Lll}{\hat \beta(\lambda)}
\newcommand{\cond}{\kappa(\lambda)}
\newcommand{\rholl}{\hat\rho_{2, \lambda}}
\newcommand{\rhowl}{\hat\rho_{1, \lambda}}
\newcommand{\supLlw}{\hat L}
\newcommand{\mufi}{\mu_\fin(\lambda)}
\newcommand{\infmufi}{\hat\mu}
\newcommand{\infq}{q}

% gd constants
\newcommand{\szc}{\alpha}
\newcommand{\sz}{\alpha(\lambda)}
\newcommand{\dsz}{\grad \alpha(\lambda)}

% ridge regression constants
\newcommand{\Lridge}{L_r(\lambda)}
\newcommand{\muridge}{\mu_r(\lambda)}
\newcommand{\Lrmin}{L}
\newcommand{\murmin}{\mu}


\newcommand{\bound}{\mathcal{B}}


%linearsystem bounds
% \newcommand{\pd}{\mu_\lambda}

\newcommand{\A}{A_\lambda}
\newcommand{\B}{b_\lambda}
\newcommand{\C}{c_\lambda}
\newcommand{\Al}{Z_\lambda}
\newcommand{\hA}{A_{\lambda,t}}
\newcommand{\hAl}{Z_{\lambda,t}}
\newcommand{\hB}{b_{\lambda,t}}
\newcommand{\hC}{c_{\lambda,t}}

\newcommand{\Z}{v(\lambda)}
\newcommand{\hZ}{v_t(\lambda)}

%approx algo iterates
\newcommand{\wo}{w_0(\lambda)}
\newcommand{\wt}{w_T(\lambda)}
\newcommand{\wT}{w_T(\lambda)}
\newcommand{\wpt}{w'_t(\lambda)}
\newcommand{\wptm}{w'_{t-1}(\lambda)}
\newcommand{\wptmm}{w'_{t-2}(\lambda)}


%fixed point/cg iterates
\newcommand{\vo}{q_{T,0}(\lambda)}
\newcommand{\vk}{q_{T,K}(\lambda)}
\newcommand{\vkm}{q_{T,K-1}(\lambda)}
\newcommand{\vkmm}{q_{T,K-2}(\lambda)}
\newcommand{\wpo}{u_{T,0}(\lambda)}
\newcommand{\wpk}{u_{T,K}(\lambda)}
\newcommand{\wpkm}{u_{T,K-1}(\lambda)}
\newcommand{\wpkmm}{u_{T,K-2}(\lambda)}


%Experiments commands
\newcommand{\Dt}{D}
\newcommand{\Dv}{D'}
\newcommand{\dist}{dist}
\newcommand{\kert}{K}
\newcommand{\kerv}{K'}
\newcommand{\Xv}{X'}
\newcommand{\Xt}{X}
\newcommand{\yt}{y}
\newcommand{\yv}{y'}


\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}


% from marthe

% \newcommand{\Prange}[2]{{P_{#1}^{#2}} }

\newcommand{\nostro}{MARTHE}  

\usepackage{tabularx}
\usepackage{booktabs}

% to add rule at the header!

\makeatletter
\newcommand{\insertheaderrule}{\rlap{\rule[-.3\normalbaselineskip]{\textwidth}{.4pt}}}
\let\old@evenhead\@evenhead \let\old@oddhead\@oddhead
\def\@evenhead{\insertheaderrule\old@evenhead}% Prepend \insertheaderrule
\def\@oddhead{\insertheaderrule\old@oddhead}% Prepend \insertheaderrule
\makeatother

% invisible sections

\newcommand\invisiblesection[1]{%
  \refstepcounter{section}%
  \addcontentsline{toc}{section}{\protect\numberline{\thesection}#1}%
  \sectionmark{#1}}


\usepackage{fixme}
\fxsetup{
    status=draft,
    author=,
    layout=inline,
    theme=color
}
% \fxsetup{theme=color}
\definecolor{fxnote}{HTML}{268bd2}
\definecolor{fxtarget}{RGB}{220,50,47}




\newcommand{\testx}{x^*}
\newcommand{\testy}{y^*}
\newcommand{\taskloss}{\mathcal{L}}
% import ---------------------- 
\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\newcommand{\ffid}[2]{f_{#2}(#1)}
\newcommand{\bmin}{b_{min}}
\newcommand{\bmax}{b_{max}}

